A Machine Learning System for Retaining Patients in HIV Care

Retaining persons living with HIV (PLWH) in medical care is paramount to preventing new transmissions of the virus and allowing PLWH to live normal and healthy lifespans. Maintaining regular appointments with an HIV provider and taking medication daily for a lifetime is exceedingly difficult. 51% of PLWH are non-adherent with their medications and eventually drop out of medical care. Current methods of re-linking individuals to care are reactive (after a patient has dropped-out) and hence not very effective. We describe our system to predict who is most at risk to drop-out-of-care for use by the University of Chicago HIV clinic and the Chicago Department of Public Health. Models were selected based on their predictive performance under resource constraints, stability over time, as well as fairness. Our system is applicable as a point-of-care system in a clinical setting as well as a batch prediction system to support regular interventions at the city level. Our model performs 3x better than the baseline for the clinical model and 2.3x better than baseline for the city-wide model. The code has been released on github and we hope this methodology, particularly our focus on fairness, will be adopted by other clinics and public health agencies in order to curb the HIV epidemic.

==> impact.tex <==
This system demonstrates the potential of machine learning models to identify individual patients at the highest risk for falling out of HIV care, allowing busy HIV care clinics to direct limited resources toward patients who need them the most. To our knowledge, this is the first use of machine learning to understand retention in care among individuals living with HIV. The system is designed to be used in both the point-of-care (at the time of patient’s appointment) and proactive outreach (generate a list of proactive intervention every month) deployment scenario. 
This system also provides tools to tune models to the resource constraints of their clinic or public health  evaluate the trade-off between performance and fairness.





 


